Network Flow Problems with Electric Vehicles

Electric vehicle (EV) adoption in long-distance logistics faces challenges such as range anxiety and uneven distribution of charging stations. Two pivotal questions emerge: How can EVs be efficiently routed in a charging network considering range limits, charging speeds and prices? And, can the existing charging infrastructure sustain the increasing demand for EVs in long-distance logistics? This paper addresses these questions by introducing a novel theoretical and computational framework to study the EV network flow problems. We present an EV network flow model that incorporates range constraints and nonlinear charging rates, and identify conditions under which polynomial-time solutions can be obtained for optimal single EV routing, maximum flow, and minimum-cost flow problems. Our findings provide insights for optimizing EV routing in logistics, ensuring an efficient and sustainable future.

==> introduction_original.tex <==
\section{Introduction}

Electric vehicle (EV) adoption for long-distance logistics faces the challenge of range anxiety. Due to the weight of the cargo and constraints on battery sizes, charging can take a considerable proportion of the trip time and requires the use of dedicated charging facilities. Additionally, the uneven distribution and limited availability of charging stations in specific regions or along certain transportation routes introduce further complications for long-distance logistics planning. Two essential questions arise: First, how to efficiently route a single EV or a fleet of EV in a charging network given the range limit, charging speed and prices? Second, given the existing charging network, what is the maximum flow that can be supported by EVs? Answering these questions is crucial for the efficient deployment of EVs in logistics services, and assessing if the current charging infrastructure can support the growing EV demand in long-distance logistics. 

To address the above-mentioned questions, we develop a theoretical and computational foundation for network flow problems with electric vehicles (EVs). Our paper make three contributions: First, we introduce an EV network flow model that incorporates range constraints and the nonlinear charging rate of charging stations. Second, we pinpoint precise conditions under which the optimal single EV routing problem, maximum flow, and minimum cost flow problems are solvable in polynomial time. Lastly, we introduce a network augmentation method that enables the efficient computation of optimal routing for both single EVs and EV fleets, as well as the maximum flow of the charging infrastructure. 



We now briefly describe our model and approach. We examine a logistics network in which a subset of nodes are equipped with electric vehicle charging stations. Chargers across different stations can vary in charging speed (e.g., DC fast chargers, level one and level two chargers). The charging speed, measured as the percentage of battery replenished over time, depends on the vehicle's current battery level — the higher the battery level, the slower the charging rate. We represent the charging speed as a piecewise linear function of the battery level. We route a fleet of electric vehicles through this network, where each vehicle has a battery range limit and is directed between a unique origin and destination. The vehicle's routing strategy specifies the chosen path and the battery charge acquired at each visited station. A charging strategy is feasible if the battery level remains within its constraints, neither depleting nor exceeding its range limit. 


Our first result focuses on determining a charging strategy for a single EV to minimize its total cost. This cost includes both the time spent on traversing edges and charging, as well as the monetary expenses associated with the charging price at each station given the acquired battery level and the price of occupying the space during the charge. In our setting, various stations and charger types can have different prices. We establish that this problem is polynomial time solvable when the shortest path measured by battery consumption between the origin and any other node is also the shortest path measured by the travel time cost (Assumption \ref{as:proportional}). If Assumption \ref{as:proportional} does not hold, the problem of optimal charging strategy reduces to a "shortest path with range constraint" problem, which is known to be NP-hard. 


Under Assumption \ref{as:proportional}, we employ a dynamic programming approach to solve the optimal charging strategy. We begin by creating an auxiliary network where each segment of the charging curve is denoted as a distinct charging station, and all stations within the battery range constraint are linked using the shortest path. We then highlight that, under the optimal charging strategy, the battery level of a vehicle upon reaching a station will fall into a finite set of values, determined by the battery capacity and the number of neighboring nodes. This property enables us to discretize the charging volume at each station without forfeiting optimality. The dynamic programming then uses a recursive approach to compute the minimal cost for vehicles transitioning from any node to the destination when the battery level corresponds to a value in the discretized set. 


We next study the problem of computing the maximum flow vector of the network subject to the capacity constraints at each charging station. This problem poses two significant hurdles: First, given that the feasible charging strategy is a vector with continuous values, the corresponding flow vector, representing the volume of the EV fleet adopting each feasible charging strategy, is infinitely dimensional. Second, as a station's charging rate is contingent on the battery level of the arriving vehicle, the station's effective capacity inherently depends on the flow vector. To navigate these challenges, we cast the maximum flow problem as a semi-infinite linear program with infinite number of variables and a finite set of constraints (\cite{LOPEZ2007491,romeijn1992duality}). Our investigation reveals that the optimal flow only takes positive value with respect to a finite set of feasible charging strategies, which are the extreme points of the feasible charging strategy set. We introduce an augmented graph, where each path represents an extreme point feasible charging strategy. Therefore, the charging network's maximum flow can be delineated as the capacity of this augmented network and solved using a finite linear program in polynomial time.




Finally, we also compute the flow vector that minimizes the total cost of routing a fleet with a fixed demand. We show that when Assumption \ref{as:proportional} holds, the computation of the minimum cost flow uses the same graph augmentation technique as the maximum flow problem, and can also be computed in polynomial time. On the other hand, without Assumption \ref{as:proportional}, the problem also becomes NP hard. 


%In this work, we develop routing algorithms for electric vehicles in a network which, in addition to taking the above factors into consideration, (1) maximize the amount of traffic that can be routed in the network, or (2) minimize the total cost (temporal and monetary) incurred by the end-users. A novelty of our model is the use of piecewise linear charging functions, which are general enough to approximate charging curves that arise in real-world instances, yet simple enough to allow for the development of polynomial-time exact algorithms. One technical challenge that arises in this setting is that, due to the continuous nature of user charging behaviours, the natural linear programming formulation of this problem is infinite-dimensional. A key insight of our algorithms is that this challenge can be circumvented by using ideas from polyhedral theory to reformulate the program as a finite (albeit exponentially-sized) LP. Moreover, there exists a polynomial-time separation oracle, and hence we are able to develop polynomial-time algorithms by appealing to the equivalence of separation and optimization. 



%We next study the problem of computing the maximum flow vector of the network subject to the capacity constraint of each charging station. The max flow computation comes with two challenges: Firstly, since the feasible charging strategy is a vector that takes continuous values, the flow vector, which indicates the volume of EV fleet to take each feasible charging strategy, has infinite dimension. Secondly, since the charging rate of each station depends on the arriving vehicle's battery level, the effective capacity of the station is endogenously depends on the flow vector. To address these two challenges, we formulate the maximum flow problem as a semi-infinite linear program with infinite number of variables and finite number of constraints. We discover that the optimal flow will only take positive value on a finite number of feasible charging strategies, which are the extreme points of the feasible charging strategy set. Then, we come up with an approach of graph-augmentation where each path of the augmented graph represents an extreme point feasible charging strategy, and thus the maximum flow of the charging network can be represented as the capacity of the augmented network, and can be solved as a finite linear program in polynomial time.   




%Our first result is to compute a charging strategy for a single EV that minimizes its total cost. Here, the cost includes the time cost of travesing edges and charging, as well as the monetary cost that includes of the price of charging at each station based on the acquired battery level and the price of occupying the space for the duration of charging time. Different stations and different types of chargers are allowed to have heterogeneous prices. We find that this problem is polynomial time solvable under the condition that the ordering of path with respect to in its length is the same as the ordering with respect to travel time.  When this condition is violated, the problem of solving the optial charging strategy reduces to a shortest path with range constraint problem, and thus becomes NP hard. We solve this problem by using a dynamic programming method. Our method involves first forming an auxiliary network, where each linear piece of the charging curve is represented as a separate charging station, and all charging stations within the battery range constraint are connected using the shortest path. Then, we demonstrate that the battery level of a vehicle when arriving at a station under the optimal charging strategy will only take a finite number of values that depends on the battery size and the number of neighbors of that node. This allows us to discretize the space of charging amount at each station without loss of optimality, and the dynamic programming takes a recursive approach to compute the minimum cost for vehicles to travel from any node to the destination when the battery level is one of such value in the discretized set. 

%We consider a logistics network, where a subset of nodes are equipped with electric vehicle charging stations. Chargers at different stations may have different charging speed (e.g. the DC fast chargers, the second and third), and the charging speed (percentage of battery provided every unit of time) depends on the battery level of the vehicle -- the higher the battery is, the slower the charger. In our setting, we assume that the charging speed is a piecewise linear function of the battery level. A fleet of Electric vehicles are routed through the network. Each vehicle has a fixed battery range constraint, and is routed between a single origin and a single destination. The routing strategy of each vehicle is the path it takes, and the amount of battery charge it gets in every visitated station. A charging strategy is feasible if the battery is never depleted and never exceeds the battery constraint. 

%Electric vehicles (EV) are a promising solution to mitigate carbon emissions. However, there are many technical challenges which must be overcome for this technology to be used in an efficient manner. In particular, there are certain problems and considerations which are unique routing EVs. For instance, EV users are more prone to \emph{range anxiety}, which refers to the user's fear of having insufficient charge (in their vehicle's battery) to complete their journey. Moreover, an EV user's refueling behaviour can deviate significantly from those of a traditional gasoline-fueled vehicle user, as recharging an EV battery can require a substantial amount of time. It is imperative that routing algorithms for electric vehicles are carefully designed, taking these factors into consideration. 

%[overview of results]
\subsection{Related literature} 
\emph{1. Shortest path and network flow algorithms.} Our problem of computing the optimal charging strategy is a natural extension of the classical shortest path problems. In classical settings, there is no constraint on the path length, and Dijkstra’s algorithm \cite{dijkstra2022note} computes the shortest path efficiently. In our problem, the cost of traversing a path needs to account for both the time cost and the battery consumption on edges, and the battery needs to be replenished before depletion at charging stations, which also incurs the cost of both time and charging prices. The optimal charging strategy computation is related to the constrained shortest path problem \cite{handler1980dual} with the goal of minimizing the total cost subject to the path length constraint. In general settings, several FPTAS algorithms have been proposed for computing the the optimal single EV charging strategy \cite{merting2015routing,baum2015shortest}.  Our analysis characterizes the condition (Assumption \ref{as:proportional}) that makes the problem solvable in polynomial time. Our dynamic programming algorithm can be viewed as an extension of the algorithm in \cite{sweda2012finding} that considered linear charging function and charge-cost only objective function, and the algorithm in \cite{khuller_fill_2007} designed for the gas filling problem. In comparison to \cite{sweda2012finding}, our algorithm incorporates the driving time cost at edges, the nonlinear charging time cost and the monetary charging cost at stations. 

Additionally, our max flow problem extends the classical max flow problem that incorporates the battery constraint and the charging capacity constraint at nodes (rather than the flow constraints on edges). Due to the inherent challenges, the classical methods \cite{ahuja1988network,ford1962flows,goldberg1988new} as well as the max-flow min-cut theorem do not readily extend to our setting. After the network augmentation procedure, our network flow problem is effectively turned into the maximum flow of the augmented network, with multiple augmented edges sharing the capacity of a single original charging station. The maximum flow of the network depends on how the station capacity is shared across different charging battery levels and charging amount that depends on the distances between a charging station and their neighbors. 




%Classical network flow is a fundamental topic in operations research, computer science, and mathematics, with numerous texts and research papers offering comprehensive insights. Ahuja, Magnanti, and Orlin's book, \cite{ahuja1993network}, is a widely acclaimed reference covering theoretical foundations, algorithms, and applications of network flows. Cormen et al.'s \cite{cormen2009introduction} "Introduction to Algorithms" includes a dedicated chapter on network flows, providing a solid introduction. Papadimitriou and Steiglitz's book \cite{papadimitriou1982combinatorial} offers a theoretical foundation for understanding flow problems. For seminal papers, Ford and Fulkerson's \cite{ford1956maximal} classic paper introduced the Ford-Fulkerson algorithm, while Goldberg and Tarjan's \cite{goldberg1988theoretical} work significantly improved algorithmic efficiency for network flow problems. These references, along with Gross and Yellen's book \cite{gross2006network}, which explores connections to network coding, collectively constitute a valuable resource for anyone studying classical network flow.

 


\emph{2. Electric vehicle routing and management.} The problem of electric vehicle routing and charging has been extensively studied in literature. One line of literature has focused on the path planning and charging problem of electric vehicle fleet in delivery problems, where the vehicles need to visit a sequence of nodes during certain time windows \cite{chen2023exponential,desaulniers2016exact,flath2014improving,kullman2021electric,froger2022electric,parmentier2023electric,sweda2017adaptive,kinay2023charging,adler2017vehicle,qi2023scaling}. This line of literature has focused on either developing heuristic approaches of path generation and charging scheduling or accelerated column generation method that solve the exact solution. Additionally, researchers have looked into the charging problem of electric robo-taxi in networked and stochastic environment using tools in stochastic optimization, fluid approximation, and deep reinforcement learning \cite{dong2022dynamic,kullman2021electric}. Moreover, the problem of infrastructure planning and battery swapping system has been investigated in \cite{mak2013infrastructure,schneider2014electric,yu2022coordinating,qi2023scaling}. Our focus is different in that we aim at developing efficient charging algorithms for long-distance logistics travel, and assess the capacity of charging network in terms of the maximum volume of EV that can be served. 


%There have been many models developed by the transportation community to address the questions of optimal electric vehicle routing and charging station placement. Some relevant recent work includes the robust optimization framework of \cite{mak2013infrastructure}, as well as many bi-level approaches (see, for instance, \cite{SHEN2019462} and the references therein) \priya{Should I give explicit reference to some of the transportation bilevel models? (e.g. Zheng et al (2017))}. The problems in theoretical computer science which are most relevant to our work are the gas station problem \cite{khuller_fill_2007}, and constrained shortest paths with resource-recovering nodes \cite{merting2015routing}. We note, however, that these models make certain assumptions that can be unrealistic in practice. 

%We now briefly comment on the literature pertaining to the theoretical techniques used in our work. The problem of routing traffic through a network is well-studied, and often tackled using techniques from the theory of network flows. As such, the algorithms we develop, and more generally, the approaches that we take, draw strong parallels from the network flows literature \cite{ford1962flows, ahuja1988network}. Another technical challenge faced when considering the EV setting is the continuous nature of users' behaviour (if one does not discretize the set of possible charge levels for the battery). %As a consequence, mathematical programming formulations in this setting can be infinite dimensional, potentially leading to a separate set of challenges (as discussed in \cite{LOPEZ2007491, romeijn1992duality}). 
